Phishing Codebook: A Structured Framework for the Characterization of Phishing Emails

Phishing is one of the most prevalent and expensive types of cybercrime faced by organizations and individuals worldwide. Most prior research has focused on various technical features and traditional representations of text to characterize phishing emails. There is a significant knowledge gap about the qualitative traits embedded in them, which could be useful in a range of phishing mitigation tasks. In this paper, we dissect the structure of phishing emails to gain a better understanding of the factors that influence human decision-making when assessing suspicious emails and identify a novel set of descriptive features. For this, we employ an iterative qualitative coding approach to identify features that are descriptive of the emails. We developed the ``Phishing Codebook'', a structured framework to systematically extract key information from phishing emails, and we apply this codebook to a publicly available dataset of 503 phishing emails collected between 2015 and 2021. We present key observations and challenges related to phishing attacks delivered indirectly through legitimate services, the challenge of recurring and long-lasting scams, and the variations within campaigns used by attackers to bypass rule-based filters. Furthermore, we provide two use cases to show how the Phishing Codebook is useful in identifying similar phishing emails and in creating well-tailored responses to end-users. We share the Phishing Codebook and the annotated benchmark dataset to help researchers have a better understanding of phishing emails.

==> parts/email-samples.tex <==
\begin{figure}[htb]
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\textwidth]{images/same_1.png} 
\caption{Email Sample 1}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\textwidth]{images/same_3.png}
\caption{Email Sample 2}
\label{fig:subim2}
\end{subfigure}
\caption{A comparison of two almost identical phishing emails sent to a user two days apart.}
\label{fig:same_ems}
\end{figure} %ORIGINAL EMLS: 2017_018, 2017_020,  2017_021

==> parts/extras.tex <==
\section{Introduction}

Phishing is a type of cyberattack in which criminals impersonate legitimate organizations and send messages via email or other means to get the user to perform an action against their best interest, such as providing their login credentials to a fraudulent website that appears to be legitimate. Phishing continues to remain a challenge partially due to the difference in how humans and computers perceive and process an email. Phishing emails often try to disguise their true source using various tricks. For instance, an email can vaguely state that it is from ``IT Services'' with the implication that it is from the organization the user works for or an email can be visual formatted to imply an email's source without ever naming the impersonated organization. These tactics are effective in deceiving humans, but they also obfuscate the implied email source from computers making it more challenging to accurately classify and cluster attacks. This study explores the use of a Qualitative Codebook to annotate phishing messages from the perspective of human interpretation. The goal is to develop a consistent framework for labeling phishing messages that can improve the composition of phishing datasets and enhance AI analysis, such as determining the cohesiveness of clusters. The proposed framework is intended to provide a better understanding of phishing attacks and improve the ability to detect and prevent them.

Phishing is an important topic to study because it is one of the most common and disruptive cyberattacks faced by organizations~\cite{cybersecurityukgov,verizon2021}. It is also one of the four most common ways to initially break into an organization~\cite{verizon2022}. The IBM Security X-Force Threat Intelligence Index 2023 states that phishing is the leading infection vector for security breaches, identified in 41\% of the incidents~\cite{ibmSecurityXForce}. Phishing attacks often result in significant financial and reputation damage to organizations and individuals alike. Given the low operational cost and high potential rewards, phishing attacks are becoming increasingly popular causing massive burden on organizations and security researchers. 

Effectively mitigating phishing attacks requires a range of interventions and a combination of technological, process, and people-based approaches~\cite{ncsc2021}, many of which can be greatly enhanced with the help of automation and AI~\cite{khonji2013}. While the automatic detection of incoming phishing emails is an important part of this defense~\cite{fette2007, benavides2020}, several other mitigation techniques require the classification of potential phishing threats into clusters. For example, some phishing emails make it past the filters, get reported by users, and then must be processed by IT staff. This can be a challenging task, particularly if there are numerous such emails to deal with~\cite{saka2022,althobaiti2021}. Clustering can also be done to understand trends over time and to gather evidence about common authors~\cite{seifollahi2017, alazab2013}. Detecting botnets or common sender sources is also important and can require emails to be clustered automatically~\cite{wei2008, han2016}. 

The evaluation of phishing email clusters is currently done either through automatically detectable features, such as URLs, or using researcher-generated labels, which often lack proper documentation. In this study, we aim to address the challenge of labeling, particularly labeling aspects of emails that require human judgment. To achieve this, we utilized a dataset of 503 publicly accessible emails that were collected over a period of seven years. We created a qualitative codebook that covers a concise set of crucial aspects of phishing emails from a human-interpretation perspective, in an iterative manner. Using a public dataset allows us to make the labels public alongside the codebook for greater transparency and replication. We also test the codebook on a different non-public dataset. The insights gained from this study can help researchers create stronger defenses against phishing attacks by combining human-like decision-making with machine capabilities. Our study aims to answer three research questions:


\begin{enumerate}
    \item[\textbf{RQ1}:] What qualitative codes would well represent the key human-interpretation features of an email?

    \item[\textbf{RQ2}:] To what extent do these qualitative codes help in identifying phishing email campaigns?
    
    \item[\textbf{RQ3}:] What kind of themes or patterns emerge from a study of phishing content?
\end{enumerate}


The remainder of this paper is organized as follows. Section~\ref{sec:bg} provides a detailed background on the topic and relevant research. Section~\ref{sec:method} describes the qualitative coding process methodology. Section~\ref{sec:results} outlines the results of the qualitative study. The main outcomes of this study are the Phishing Codebook and coded dataset, which we explain in detail in Section~\ref{sec:codebook}. We also present our findings regarding the various trends that emerged from the coded datasets. Section~\ref{sec:app1} outlines our experiment and describes the use of qualitative attributes for campaign detection. In Section~\ref{sec:disscussion}, we discuss some of the potential applications of the Phishing Codebook and some limitations of this study. Finally, Section~\ref{sec:conc} provides the conclusions of our study and directions for future work.


